Is forgetting less a good inductive bias for forward transfer?

One of the main motivations of studying continual learning is that the problem setting allows a model to accrue knowledge from past tasks to learn new tasks more efficiently. However, recent studies suggest that the key metric that continual learning algorithms optimize, reduction in catastrophic forgetting, does not correlate well with the forward transfer of knowledge. We believe that the conclusion previous works reached is due to the way they measure forward transfer. We argue that the measure of forward transfer to a task should not be affected by the restrictions placed on the continual learner in order to preserve knowledge of previous tasks. Instead, forward transfer should be measured by how easy it is to learn a new task given a set of representations produced by continual learning on previous tasks. Under this notion of forward transfer, we evaluate different continual learning algorithms on a variety of image classification benchmarks. Our results indicate that less forgetful representations lead to a better forward transfer suggesting a strong correlation between retaining past information and learning efficiency on new tasks. Further, we found less forgetful representations to be more diverse and discriminative compared to their forgetful counterparts.

==> backup.tex <==
\newpage

% \subsection{Correlation Measurement}


% \begin{table*}[htb]
%     \centering
%     % \begin{adjustbox}{width=\columnwidth,center}
% 		\begin{tabular}{l|ccc|ccc}
% 			\toprule
% 			  \multirow{2}{0.12\linewidth}{Dataset} &  \multicolumn{3}{c|}{Random Init} & \multicolumn{3}{c}{Pretrain}  \\ \cline{2-7}
% 			  & $k=5$ & $k=10$ & $k=20$  & $k=5$ & $k=10$ & $k=20$  \\ \hline
% 			 Split CIFAR-10 & 0.4713 & 0.4143 & 0.5218 & 0.4419 & 0.3425 & 0.3333 \\
% 			\bottomrule
% 		\end{tabular}
% % 	\end{adjustbox}
% 	\caption[]{\small  Kendall’s tau between $\avgfgt$ and $\avgfwt$ for different $k$. }
% 	\label{tab:correlation-results}
% \end{table*}

\begin{table*}[htb]
    \centering
    % \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c|}{Random Init} & \multicolumn{2}{c}{Pretrain}  \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfwt(k=5)$  &  $\avgfgt$ & $\avgfwt(k=5)$  \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
			 & FT & -28.18 $\pm$ 2.39 & 61.95 $\pm$ 1.45 & -29.01 $\pm$ 6.42 & 66.15 $\pm$ 2.91   \\
            & LP-FT & -29.50 $\pm$ 4.67 & 61.96 $\pm$ 3.28 & -3.39 $\pm$ 0.85 & 73.04 $\pm$ 1.66  \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & 62.72 $\pm$ 1.68 & -7.15 $\pm$ 1.59 & 67.62 $\pm$ 4.39   \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & 61.05 $\pm$ 1.13 & -19.26 $\pm$ 4.04 & 64.32 $\pm$ 2.69  \\
            & MT & -3.88 $\pm$ 4.72 & 64.60 $\pm$ 0.85 & -4.83 $\pm$ 4.48 & 70.68 $\pm$ 1.71   \\
            & FOMAML & -0.75 $\pm$ 1.12 & 65.47 $\pm$ 1.34 & -1.40 $\pm$ 0.49 & 70.18 $\pm$ 2.47   \\ \hline
			  \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 & FT & -25.83 $\pm$ 1.96 & 52.32 $\pm$ 0.43 & -24.33 $\pm$ 3.38 & 60.43 $\pm$ 1.60   \\
            & LP-FT & -23.93 $\pm$ 7.09 & 51.77 $\pm$ 1.05 & -4.46 $\pm$ 0.37 & 68.65 $\pm$ 0.93   \\
            & ER (m=20) & -9.44 $\pm$ 0.89 & 53.74 $\pm$ 0.60 & -9.19 $\pm$ 0.23 & 64.04 $\pm$ 0.13   \\
            & AGEM (m=20) & -18.70 $\pm$ 0.80 & 52.52 $\pm$ 0.58 & -20.05 $\pm$ 2.52 & 60.31 $\pm$ 1.99   \\
            & MT & -9.35 $\pm$ 3.99 & 53.60 $\pm$ 0.88 & -7.93 $\pm$ 3.26 & 64.27 $\pm$ 0.81   \\
            & FOMAML & -3.05 $\pm$ 0.79 & 55.65 $\pm$ 0.76 & -4.40 $\pm$ 0.16 & 64.83 $\pm$ 1.05   \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
			 & FT & -14.45 $\pm$ 0.82 & 31.98 $\pm$ 1.01 & -13.51 $\pm$ 0.45 & 47.69 $\pm$ 1.27   \\
            & LP-FT & -8.50 $\pm$ 0.76 & 31.13 $\pm$ 1.02 & -2.66 $\pm$ 0.43 & 49.58 $\pm$ 0.49   \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & 31.76 $\pm$ 1.00 & -11.36 $\pm$ 1.16 & 47.78 $\pm$ 1.38   \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & 32.01 $\pm$ 0.60 & -12.11 $\pm$ 0.61 & 47.49 $\pm$ 1.08   \\
            & MT & -1.30 $\pm$ 3.24 & 32.36 $\pm$ 0.73 & -5.50 $\pm$ 2.94 & 48.35 $\pm$ 0.31   \\
            & FOMAML & 1.99 $\pm$ 0.61 & 33.63 $\pm$ 1.04 & -1.24 $\pm$ 0.35 & 48.23 $\pm$ 0.72   \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & 56.38 $\pm$ 0.74 & 0.14 $\pm$ 0.34 & 90.45 $\pm$ 0.14  \\
            & LP-FT & 1.18 $\pm$ 0.52 & 56.71 $\pm$ 0.22 & 0.87 $\pm$ 0.09 & 90.46 $\pm$ 0.09  \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & 56.81 $\pm$ 0.40 & -0.05 $\pm$ 0.18 & 90.59 $\pm$ 0.20   \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & 56.33 $\pm$ 0.96 & -0.01 $\pm$ 0.15 & 90.38 $\pm$ 0.10   \\
            & MT & 4.49 $\pm$ 0.80 & 58.65 $\pm$ 0.61 & 0.77 $\pm$ 0.41 & 91.29 $\pm$ 0.41   \\
            & FOMAML & 4.49 $\pm$ 0.45 & 60.38 $\pm$ 0.82 & 0.84 $\pm$ 0.27 & 91.20 $\pm$ 0.23  \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
			 & FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
            & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
            & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
            & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
            & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
            & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
% 	\end{adjustbox}
	\caption[]{\small All numbers are percentages. }
	\label{tab:main-results}
\end{table*}



\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|ccccc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{5}{c}{Random Init}   \\ \cline{3-7}
			  & & $\avgfgt$ & $\avgfwt(k=5)$  & Feature Score & Feature Score 1 &  Feature Score 2 \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
			 & FT & -28.18 $\pm$ 2.39 & 64.11 $\pm$ 2.06 & -1.49 $\pm$ 0.42 & 44.97 $\pm$ 3.88 & 46.47 $\pm$ 3.51 \\
& LP-FT & -29.50 $\pm$ 4.67 & 64.13 $\pm$ 4.35 & -2.02 $\pm$ 0.97 & 35.17 $\pm$ 8.72 & 37.19 $\pm$ 7.79 \\
& ER (m=50) & -9.18 $\pm$ 1.20 & 65.08 $\pm$ 2.42 & -1.41 $\pm$ 0.31 & 51.24 $\pm$ 2.26 & 52.65 $\pm$ 1.98 \\
& AGEM (m=50) & -13.77 $\pm$ 1.92 & 62.99 $\pm$ 1.79 & -1.33 $\pm$ 0.34 & 48.64 $\pm$ 4.63 & 49.97 $\pm$ 4.35 \\
& MT & -3.88 $\pm$ 4.72 & 67.43 $\pm$ 1.08 & -1.26 $\pm$ 0.32 & 47.77 $\pm$ 5.41 & 49.04 $\pm$ 5.13 \\
& FOMAML & -0.75 $\pm$ 1.12 & 68.52 $\pm$ 1.88 & -1.17 $\pm$ 0.39 & 51.42 $\pm$ 1.53 & 52.59 $\pm$ 1.19 \\ \hline
			 % \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 %& FT & -25.83 $\pm$ 1.96 & 52.32 $\pm$ 0.43 & -24.33 $\pm$ 3.38 & 60.43 $\pm$ 1.60   \\
    %         & LP-FT & -23.93 $\pm$ 7.09 & 51.77 $\pm$ 1.05 & -4.46 $\pm$ 0.37 & 68.65 $\pm$ 0.93   \\
    %         & ER (m=20) & -9.44 $\pm$ 0.89 & 53.74 $\pm$ 0.60 & -9.19 $\pm$ 0.23 & 64.04 $\pm$ 0.13   \\
    %         & AGEM (m=20) & -18.70 $\pm$ 0.80 & 52.52 $\pm$ 0.58 & -20.05 $\pm$ 2.52 & 60.31 $\pm$ 1.99   \\
    %         & MT & -9.35 $\pm$ 3.99 & 53.60 $\pm$ 0.88 & -7.93 $\pm$ 3.26 & 64.27 $\pm$ 0.81   \\
    %         & FOMAML & -3.05 $\pm$ 0.79 & 55.65 $\pm$ 0.76 & -4.40 $\pm$ 0.16 & 64.83 $\pm$ 1.05   \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
			 & FT & -14.45 $\pm$ 0.82 & 37.85 $\pm$ 1.33 & -44.95 $\pm$ 2.08 & 616.96 $\pm$ 3.74 & 661.90 $\pm$ 2.80 \\
& LP-FT & -8.50 $\pm$ 0.76 & 36.79 $\pm$ 1.40 & -46.01 $\pm$ 1.24 & 615.98 $\pm$ 1.51 & 661.99 $\pm$ 0.54 \\
& ER (m=5) & -11.33 $\pm$ 1.44 & 37.57 $\pm$ 1.29 & -44.57 $\pm$ 1.77 & 616.74 $\pm$ 2.34 & 661.31 $\pm$ 1.38 \\
& AGEM (m=5) & -12.28 $\pm$ 0.67 & 37.88 $\pm$ 0.81 & -45.03 $\pm$ 1.81 & 616.07 $\pm$ 3.30 & 661.10 $\pm$ 2.08 \\
& MT & -1.30 $\pm$ 3.24 & 38.33 $\pm$ 0.94 & -43.89 $\pm$ 1.92 & 619.30 $\pm$ 2.89 & 663.19 $\pm$ 1.80 \\
& FOMAML & 1.99 $\pm$ 0.61 & 39.92 $\pm$ 1.36 & -43.58 $\pm$ 1.10 & 622.67 $\pm$ 1.79 & 666.25 $\pm$ 0.99 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & 60.29 $\pm$ 0.77 & -52.07 $\pm$ 0.79 & 178.05 $\pm$ 1.25 & 230.12 $\pm$ 1.01 \\
& LP-FT & 1.18 $\pm$ 0.52 & 60.65 $\pm$ 0.25 & -52.88 $\pm$ 0.97 & 183.68 $\pm$ 1.60 & 236.56 $\pm$ 1.71 \\
& ER (m=10) & 1.79 $\pm$ 0.19 & 60.77 $\pm$ 0.40 & -51.70 $\pm$ 0.93 & 178.15 $\pm$ 1.52 & 229.85 $\pm$ 1.04 \\
& AGEM (m=10) & 2.03 $\pm$ 0.69 & 60.24 $\pm$ 1.04 & -52.32 $\pm$ 0.69 & 177.08 $\pm$ 1.55 & 229.40 $\pm$ 1.27 \\
& MT & 4.49 $\pm$ 0.80 & 62.82 $\pm$ 0.71 & -49.93 $\pm$ 0.75 & 178.29 $\pm$ 0.58 & 228.22 $\pm$ 0.51 \\
& FOMAML & 4.49 $\pm$ 0.45 & 64.74 $\pm$ 0.94 & -50.83 $\pm$ 0.43 & 180.05 $\pm$ 1.24 & 230.88 $\pm$ 1.00 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
			& FT & 5.06 $\pm$ 0.23 & 30.43 $\pm$ 0.33 & -1004.70 $\pm$ 2.17 & 1643.04 $\pm$ 4.95 & 2647.74 $\pm$ 3.01 \\
& LP-FT & 5.13 $\pm$ 0.47 & 31.85 $\pm$ 0.32 & -990.36 $\pm$ 2.03 & 1790.63 $\pm$ 2.15 & 2780.98 $\pm$ 3.06 \\
& ER (m=5) & 5.53 $\pm$ 0.19 & 30.32 $\pm$ 0.32 & -997.26 $\pm$ 4.07 & 1654.94 $\pm$ 7.26 & 2652.20 $\pm$ 3.35 \\
& AGEM (m=5) & 4.94 $\pm$ 0.29 & 30.25 $\pm$ 0.32 & -1007.19 $\pm$ 1.65 & 1641.99 $\pm$ 2.54 & 2649.17 $\pm$ 2.54 \\
& MT & 8.65 $\pm$ 0.78 & 34.01 $\pm$ 0.61 & -973.90 $\pm$ 3.34 & 1680.07 $\pm$ 20.73 & 2653.97 $\pm$ 18.66 \\
& FOMAML & 9.21 $\pm$ 0.10 & 35.17 $\pm$ 0.41 & -981.69 $\pm$ 3.41 & 1709.01 $\pm$ 6.06 & 2690.70 $\pm$ 4.34 \\ \hline
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Except Feature Score, all numbers are percentages. }
	\label{tab:feature-score-random-init-results}
\end{table*}


\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|ccccc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{5}{c}{Pre-trained}   \\ \cline{3-7}
			  & & $\avgfgt$ & $\avgfwt(k=5)$  & Feature Score & Feature Score 1 &  Feature Score 2 \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
			& FT & -29.01 $\pm$ 6.42 & 64.61 $\pm$ 3.20 & -0.78 $\pm$ 0.71 & 42.11 $\pm$ 15.85 & 42.89 $\pm$ 15.20 \\
& LP-FT & -3.39 $\pm$ 0.85 & 73.22 $\pm$ 1.30 & -0.19 $\pm$ 0.06 & 68.52 $\pm$ 1.24 & 68.70 $\pm$ 1.25 \\
& ER (m=50) & -7.15 $\pm$ 1.59 & 66.44 $\pm$ 4.01 & -0.76 $\pm$ 0.43 & 49.90 $\pm$ 5.94 & 50.66 $\pm$ 5.55 \\
& AGEM (m=50) & -19.26 $\pm$ 4.04 & 62.32 $\pm$ 1.27 & -1.12 $\pm$ 1.43 & 42.30 $\pm$ 13.04 & 43.42 $\pm$ 11.72 \\
& MT & -4.83 $\pm$ 4.48 & 70.26 $\pm$ 2.86 & -0.37 $\pm$ 0.21 & 52.27 $\pm$ 5.04 & 52.63 $\pm$ 4.91 \\
& FOMAML & -1.40 $\pm$ 0.49 & 69.65 $\pm$ 3.40 & -0.57 $\pm$ 0.13 & 49.55 $\pm$ 4.04 & 50.12 $\pm$ 4.05 \\ \hline
			 % \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 %& FT & -25.83 $\pm$ 1.96 & 52.32 $\pm$ 0.43 & -24.33 $\pm$ 3.38 & 60.43 $\pm$ 1.60   \\
    %         & LP-FT & -23.93 $\pm$ 7.09 & 51.77 $\pm$ 1.05 & -4.46 $\pm$ 0.37 & 68.65 $\pm$ 0.93   \\
    %         & ER (m=20) & -9.44 $\pm$ 0.89 & 53.74 $\pm$ 0.60 & -9.19 $\pm$ 0.23 & 64.04 $\pm$ 0.13   \\
    %         & AGEM (m=20) & -18.70 $\pm$ 0.80 & 52.52 $\pm$ 0.58 & -20.05 $\pm$ 2.52 & 60.31 $\pm$ 1.99   \\
    %         & MT & -9.35 $\pm$ 3.99 & 53.60 $\pm$ 0.88 & -7.93 $\pm$ 3.26 & 64.27 $\pm$ 0.81   \\
    %         & FOMAML & -3.05 $\pm$ 0.79 & 55.65 $\pm$ 0.76 & -4.40 $\pm$ 0.16 & 64.83 $\pm$ 1.05   \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
			& FT & -13.51 $\pm$ 0.45 & 49.46 $\pm$ 2.06 & -22.81 $\pm$ 2.45 & 671.77 $\pm$ 2.67 & 694.58 $\pm$ 2.22 \\
& LP-FT & -2.66 $\pm$ 0.43 & 51.82 $\pm$ 1.13 & -17.51 $\pm$ 1.41 & 715.83 $\pm$ 4.64 & 733.34 $\pm$ 6.04 \\
& ER (m=5) & -11.36 $\pm$ 1.16 & 49.58 $\pm$ 2.15 & -23.11 $\pm$ 2.36 & 676.84 $\pm$ 3.88 & 699.95 $\pm$ 3.98 \\
& AGEM (m=5) & -12.11 $\pm$ 0.61 & 49.21 $\pm$ 1.82 & -23.15 $\pm$ 2.13 & 671.65 $\pm$ 5.44 & 694.81 $\pm$ 3.97 \\
& MT & -5.50 $\pm$ 2.94 & 50.29 $\pm$ 0.84 & -22.45 $\pm$ 2.07 & 675.17 $\pm$ 6.34 & 697.62 $\pm$ 4.41 \\
& FOMAML & -1.24 $\pm$ 0.35 & 50.14 $\pm$ 1.23 & -22.15 $\pm$ 1.96 & 691.28 $\pm$ 4.22 & 713.43 $\pm$ 2.99 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.14 $\pm$ 0.34 & 91.67 $\pm$ 0.16 & -9.95 $\pm$ 0.12 & 281.79 $\pm$ 0.62 & 291.74 $\pm$ 0.62 \\
& LP-FT & 0.87 $\pm$ 0.09 & 91.68 $\pm$ 0.10 & -8.93 $\pm$ 0.13 & 284.97 $\pm$ 0.50 & 293.89 $\pm$ 0.57 \\
& ER (m=10) & -0.05 $\pm$ 0.18 & 91.83 $\pm$ 0.22 & -9.86 $\pm$ 0.17 & 281.71 $\pm$ 0.48 & 291.57 $\pm$ 0.33 \\
& AGEM (m=10) & -0.01 $\pm$ 0.15 & 91.60 $\pm$ 0.11 & -9.92 $\pm$ 0.18 & 282.24 $\pm$ 0.73 & 292.17 $\pm$ 0.81 \\
& MT & 0.77 $\pm$ 0.41 & 92.61 $\pm$ 0.45 & -9.83 $\pm$ 0.12 & 282.18 $\pm$ 0.78 & 292.01 $\pm$ 0.68 \\
& FOMAML & 0.84 $\pm$ 0.27 & 92.50 $\pm$ 0.26 & -10.15 $\pm$ 0.12 & 281.55 $\pm$ 0.89 & 291.69 $\pm$ 0.96 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
			& FT & -0.03 $\pm$ 0.11 & 81.13 $\pm$ 0.13 & -461.37 $\pm$ 1.14 & 2505.80 $\pm$ 2.68 & 2967.17 $\pm$ 2.76 \\
& LP-FT & 1.52 $\pm$ 0.06 & 83.59 $\pm$ 0.04 & -389.08 $\pm$ 1.34 & 2587.60 $\pm$ 2.46 & 2976.68 $\pm$ 2.00 \\
& ER (m=5) & 0.34 $\pm$ 0.14 & 81.60 $\pm$ 0.10 & -458.02 $\pm$ 2.43 & 2504.28 $\pm$ 3.08 & 2962.30 $\pm$ 3.71 \\
& AGEM (m=5) & 0.04 $\pm$ 0.11 & 81.10 $\pm$ 0.05 & -460.48 $\pm$ 2.27 & 2506.17 $\pm$ 2.87 & 2966.65 $\pm$ 4.16 \\
& MT & 1.56 $\pm$ 0.12 & 83.51 $\pm$ 0.11 & -449.37 $\pm$ 1.48 & 2492.15 $\pm$ 4.36 & 2941.52 $\pm$ 5.40 \\
& FOMAML & 1.55 $\pm$ 0.13 & 83.35 $\pm$ 0.15 & -453.85 $\pm$ 2.70 & 2483.20 $\pm$ 2.08 & 2937.05 $\pm$ 4.15 \\ \hline

    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Except Feature Score, all numbers are percentages. }
	\label{tab:feature-score-pretrain-results}
\end{table*}


\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|ccccc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{5}{c}{Random Init}   \\ \cline{3-7}
			  & & $\avgfgt$ & $\avgfwt(k=5)$  & Feature Score & Feature Score 1 &  Feature Score 2 \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
			 & FT & -28.18 $\pm$ 2.39 & 64.11 $\pm$ 2.06 & -2.95 $\pm$ 0.92 & 84.89 $\pm$ 7.87 & 87.84 $\pm$ 7.34 \\
& LP-FT & -29.50 $\pm$ 4.67 & 64.13 $\pm$ 4.35 & -4.04 $\pm$ 1.70 & 63.50 $\pm$ 19.89 & 67.54 $\pm$ 18.42 \\
& ER (m=50) & -9.18 $\pm$ 1.20 & 65.08 $\pm$ 2.42 & -2.86 $\pm$ 1.10 & 96.07 $\pm$ 2.49 & 98.93 $\pm$ 2.66 \\
& AGEM (m=50) & -13.77 $\pm$ 1.92 & 62.99 $\pm$ 1.79 & -2.61 $\pm$ 1.14 & 90.96 $\pm$ 6.56 & 93.57 $\pm$ 5.64 \\
& MT & -3.88 $\pm$ 4.72 & 67.43 $\pm$ 1.08 & -2.59 $\pm$ 0.93 & 89.84 $\pm$ 7.82 & 92.43 $\pm$ 6.91 \\
& FOMAML & -0.75 $\pm$ 1.12 & 68.52 $\pm$ 1.88 & -2.55 $\pm$ 0.93 & 98.47 $\pm$ 5.35 & 101.02 $\pm$ 4.44 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
			& FT & -14.45 $\pm$ 0.82 & 37.85 $\pm$ 1.33 & -101.46 $\pm$ 10.67 & 1192.86 $\pm$ 9.80 & 1294.32 $\pm$ 3.28 \\
& LP-FT & -8.50 $\pm$ 0.76 & 36.79 $\pm$ 1.40 & -106.72 $\pm$ 7.29 & 1191.14 $\pm$ 6.20 & 1297.86 $\pm$ 1.68 \\
& ER (m=5) & -11.33 $\pm$ 1.44 & 37.57 $\pm$ 1.29 & -101.42 $\pm$ 9.93 & 1193.62 $\pm$ 7.01 & 1295.04 $\pm$ 4.83 \\
& AGEM (m=5) & -12.28 $\pm$ 0.67 & 37.88 $\pm$ 0.81 & -101.91 $\pm$ 10.20 & 1192.28 $\pm$ 9.43 & 1294.19 $\pm$ 1.12 \\
& MT & -1.30 $\pm$ 3.24 & 38.33 $\pm$ 0.94 & -100.04 $\pm$ 10.09 & 1197.77 $\pm$ 9.82 & 1297.80 $\pm$ 4.42 \\
& FOMAML & 1.99 $\pm$ 0.61 & 39.92 $\pm$ 1.36 & -100.66 $\pm$ 8.07 & 1205.14 $\pm$ 5.60 & 1305.80 $\pm$ 3.70 \\ \hline
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Compute scores using train features. Except Feature Score, all numbers are percentages. }
	\label{tab:feature-score-random-init-results}
\end{table*}


\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|ccccc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{5}{c}{Pre-trained}   \\ \cline{3-7}
			  & & $\avgfgt$ & $\avgfwt(k=5)$  & Feature Score & Feature Score 1 &  Feature Score 2 \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
		      & FT & -29.01 $\pm$ 6.42 & 64.61 $\pm$ 3.20 & -4.39 $\pm$ 6.04 & 73.73 $\pm$ 44.41 & 78.12 $\pm$ 38.40 \\
& LP-FT & -3.39 $\pm$ 0.85 & 73.22 $\pm$ 1.30 & -0.51 $\pm$ 0.14 & 138.56 $\pm$ 1.44 & 139.07 $\pm$ 1.32 \\
& ER (m=50) & -7.15 $\pm$ 1.59 & 66.44 $\pm$ 4.01 & -1.95 $\pm$ 1.16 & 95.42 $\pm$ 13.79 & 97.37 $\pm$ 12.71 \\
& AGEM (m=50) & -19.26 $\pm$ 4.04 & 62.32 $\pm$ 1.27 & -2.85 $\pm$ 2.56 & 80.12 $\pm$ 29.75 & 82.96 $\pm$ 27.26 \\
& MT & -4.83 $\pm$ 4.48 & 70.26 $\pm$ 2.86 & -1.27 $\pm$ 0.77 & 101.22 $\pm$ 9.65 & 102.48 $\pm$ 8.98 \\
& FOMAML & -1.40 $\pm$ 0.49 & 69.65 $\pm$ 3.40 & -1.62 $\pm$ 0.94 & 95.90 $\pm$ 6.76 & 97.52 $\pm$ 7.10 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
			& FT & -13.51 $\pm$ 0.45 & 49.46 $\pm$ 2.06 & -60.52 $\pm$ 9.45 & 1308.69 $\pm$ 6.29 & 1369.20 $\pm$ 7.79 \\
& LP-FT & -2.66 $\pm$ 0.43 & 51.82 $\pm$ 1.13 & -46.22 $\pm$ 5.33 & 1409.84 $\pm$ 7.05 & 1456.05 $\pm$ 12.32 \\
& ER (m=5) & -11.36 $\pm$ 1.16 & 49.58 $\pm$ 2.15 & -61.70 $\pm$ 8.01 & 1316.90 $\pm$ 8.50 & 1378.61 $\pm$ 10.59 \\
& AGEM (m=5) & -12.11 $\pm$ 0.61 & 49.21 $\pm$ 1.82 & -60.65 $\pm$ 8.79 & 1308.95 $\pm$ 10.39 & 1369.60 $\pm$ 5.56 \\
& MT & -5.50 $\pm$ 2.94 & 50.29 $\pm$ 0.84 & -60.02 $\pm$ 8.75 & 1316.42 $\pm$ 13.22 & 1376.45 $\pm$ 5.35 \\
& FOMAML & -1.24 $\pm$ 0.35 & 50.14 $\pm$ 1.23 & -58.67 $\pm$ 7.92 & 1348.88 $\pm$ 9.88 & 1407.55 $\pm$ 5.91 \\ \hline
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Compute scores using train features. Except Feature Score, all numbers are percentages. }
	\label{tab:feature-score-pretrain-results}
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
			& FT & -28.18 $\pm$ 2.39 & -1.49 $\pm$ 0.42 & -29.01 $\pm$ 6.42 & -0.78 $\pm$ 0.71 \\
            & LP-FT & - & - &  -3.39 $\pm$ 0.85 & {\bf -0.19} $\pm$ 0.06 \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & -1.41 $\pm$ 0.31 & -7.15 $\pm$ 1.59 & -0.76 $\pm$ 0.43 \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & -1.33 $\pm$ 0.34 & -19.26 $\pm$ 4.04 & -1.12 $\pm$ 1.43 \\
            & MT & -3.88 $\pm$ 4.72 & -1.26 $\pm$ 0.32 & -4.83 $\pm$ 4.48 & -0.37 $\pm$ 0.21 \\
            & FOMAML & {\bf -0.75} $\pm$ 1.12 & {\bf -1.17} $\pm$ 0.39 & -1.40 $\pm$ 0.49 & -0.57 $\pm$ 0.13 \\ \hline
			 % \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 %& FT & -25.83 $\pm$ 1.96 & 52.32 $\pm$ 0.43 & -24.33 $\pm$ 3.38 & 60.43 $\pm$ 1.60   \\
    %         & LP-FT & -23.93 $\pm$ 7.09 & 51.77 $\pm$ 1.05 & -4.46 $\pm$ 0.37 & 68.65 $\pm$ 0.93   \\
    %         & ER (m=20) & -9.44 $\pm$ 0.89 & 53.74 $\pm$ 0.60 & -9.19 $\pm$ 0.23 & 64.04 $\pm$ 0.13   \\
    %         & AGEM (m=20) & -18.70 $\pm$ 0.80 & 52.52 $\pm$ 0.58 & -20.05 $\pm$ 2.52 & 60.31 $\pm$ 1.99   \\
    %         & MT & -9.35 $\pm$ 3.99 & 53.60 $\pm$ 0.88 & -7.93 $\pm$ 3.26 & 64.27 $\pm$ 0.81   \\
    %         & FOMAML & -3.05 $\pm$ 0.79 & 55.65 $\pm$ 0.76 & -4.40 $\pm$ 0.16 & 64.83 $\pm$ 1.05   \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
			& FT & -14.45 $\pm$ 0.82 & -44.95 $\pm$ 2.08 & -13.51 $\pm$ 0.45 & -22.81 $\pm$ 2.45 \\
            & LP-FT & - & - &  -2.66 $\pm$ 0.43 & {\bf -17.51} $\pm$ 1.41 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & -44.57 $\pm$ 1.77 & -11.36 $\pm$ 1.16 & -23.11 $\pm$ 2.36 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & -45.03 $\pm$ 1.81 & -12.11 $\pm$ 0.61 & -23.15 $\pm$ 2.13 \\
            & MT & -1.30 $\pm$ 3.24 & -43.89 $\pm$ 1.92 & -5.50 $\pm$ 2.94 & -22.45 $\pm$ 2.07 \\
            & FOMAML & {\bf 1.99} $\pm$ 0.61 & {\bf -43.58} $\pm$ 1.10 & -1.24 $\pm$ 0.35 & -22.15 $\pm$ 1.96 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & -52.07 $\pm$ 0.79 & 0.14 $\pm$ 0.34 & -9.95 $\pm$ 0.12 \\
            & LP-FT & - & - & 0.87 $\pm$ 0.09 & {\bf -8.93} $\pm$ 0.13 \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & -51.70 $\pm$ 0.93 & -0.05 $\pm$ 0.18 & -9.86 $\pm$ 0.17 \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & -52.32 $\pm$ 0.69 & -0.01 $\pm$ 0.15 & -9.92 $\pm$ 0.18 \\
            & MT & {\bf 4.49} $\pm$ 0.80 & {\bf -49.93} $\pm$ 0.75 & 0.77 $\pm$ 0.41 & -9.83 $\pm$ 0.12 \\
            & FOMAML & {\bf 4.49} $\pm$ 0.45 & -50.83 $\pm$ 0.43 & 0.84 $\pm$ 0.27 & -10.15 $\pm$ 0.12 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
		    & FT & 5.06 $\pm$ 0.23 & -1004.70 $\pm$ 2.17 & -0.03 $\pm$ 0.11 & -461.37 $\pm$ 1.14 \\
            & LP-FT & - & -  & 1.52 $\pm$ 0.06 & {\bf -389.08} $\pm$ 1.34 \\
            & ER (m=5) & 5.53 $\pm$ 0.19 & -997.26 $\pm$ 4.07 & 0.34 $\pm$ 0.14 & -458.02 $\pm$ 2.43 \\
            & AGEM (m=5) & 4.94 $\pm$ 0.29 & -1007.19 $\pm$ 1.65 & 0.04 $\pm$ 0.11 & -460.48 $\pm$ 2.27 \\
            & MT & 8.65 $\pm$ 0.78 & {\bf -973.90} $\pm$ 3.34 & 1.56 $\pm$ 0.12 & -449.37 $\pm$ 1.48 \\
            & FOMAML & {\bf 9.21} $\pm$ 0.10 & -981.69 $\pm$ 3.41 & 1.55 $\pm$ 0.13 & -453.85 $\pm$ 2.70 \\ \hline
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v1-results}
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
    		& FT & -28.18 $\pm$ 2.39 & 2684.86 $\pm$ 809.58 & -29.01 $\pm$ 6.42 & -2742.99 $\pm$ 10118.58 \\
            & LP-FT &  - & - &  -3.39 $\pm$ 0.85 & {\bf 10101.57} $\pm$ 223.25 \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & 3939.22 $\pm$ 178.04 & -7.15 $\pm$ 1.59 & 774.75 $\pm$ 3390.75 \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & 3402.46 $\pm$ 869.99 & -19.26 $\pm$ 4.04 & -3638.12 $\pm$ 10804.17 \\
            & MT & -3.88 $\pm$ 4.72 & 3476.90 $\pm$ 837.50 & -4.83 $\pm$ 4.48 & 3369.75 $\pm$ 1726.75 \\
            & FOMAML & {\bf -0.75} $\pm$ 1.12 & {\bf 4444.74} $\pm$ 434.90 & {\bf -1.40 $\pm$ 0.49} & 828.85 $\pm$ 2765.08 \\ \hline
			 % \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 %& FT & -25.83 $\pm$ 1.96 & 52.32 $\pm$ 0.43 & -24.33 $\pm$ 3.38 & 60.43 $\pm$ 1.60   \\
    %         & LP-FT & -23.93 $\pm$ 7.09 & 51.77 $\pm$ 1.05 & -4.46 $\pm$ 0.37 & 68.65 $\pm$ 0.93   \\
    %         & ER (m=20) & -9.44 $\pm$ 0.89 & 53.74 $\pm$ 0.60 & -9.19 $\pm$ 0.23 & 64.04 $\pm$ 0.13   \\
    %         & AGEM (m=20) & -18.70 $\pm$ 0.80 & 52.52 $\pm$ 0.58 & -20.05 $\pm$ 2.52 & 60.31 $\pm$ 1.99   \\
    %         & MT & -9.35 $\pm$ 3.99 & 53.60 $\pm$ 0.88 & -7.93 $\pm$ 3.26 & 64.27 $\pm$ 0.81   \\
    %         & FOMAML & -3.05 $\pm$ 0.79 & 55.65 $\pm$ 0.76 & -4.40 $\pm$ 0.16 & 64.83 $\pm$ 1.05   \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
			& FT & -14.45 $\pm$ 0.82 & 8359.15 $\pm$ 62.54 & -13.51 $\pm$ 0.45 & 9438.93 $\pm$ 82.78 \\
            & LP-FT & - & -  & -2.66 $\pm$ 0.43 & {\bf 10843.78} $\pm$ 99.82 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & 8351.30 $\pm$ 42.58 & -11.36 $\pm$ 1.16 & 9518.64 $\pm$ 147.85 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & 8339.23 $\pm$ 51.05 & -12.11 $\pm$ 0.61 & 9428.18 $\pm$ 73.79 \\
            & MT & -1.30 $\pm$ 3.24 & 8404.61 $\pm$ 51.80 & -5.50 $\pm$ 2.94 & 9509.01 $\pm$ 89.57 \\
            & FOMAML & {\bf 1.99} $\pm$ 0.61 & {\bf 8426.69} $\pm$ 27.71 & {\bf -1.24} $\pm$ 0.35 & 9911.71 $\pm$ 90.23 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & -11588.13 $\pm$ 24.09 & 0.14 $\pm$ 0.34 & -10846.96 $\pm$ 28.30 \\
            & LP-FT & - & -  & {\bf 0.87} $\pm$ 0.09 & {\bf -10723.84} $\pm$ 15.55 \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & -11582.33 $\pm$ 10.76 & -0.05 $\pm$ 0.18 & -10831.29 $\pm$ 20.83 \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & -11598.41 $\pm$ 23.61 & -0.01 $\pm$ 0.15 & -10849.51 $\pm$ 11.56 \\
            & MT & {\bf 4.49} $\pm$ 0.80 & -11544.05 $\pm$ 19.04 & 0.77 $\pm$ 0.41 & -10800.50 $\pm$ 33.86 \\
            & FOMAML & {\bf 4.49} $\pm$ 0.45 & {\bf -11501.26} $\pm$ 11.54 & 0.84 $\pm$ 0.27 & -10804.14 $\pm$ 22.46 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
		    & FT & 5.06 $\pm$ 0.23 & 7030.61 $\pm$ 22.34 & -0.03 $\pm$ 0.11 & 10423.92 $\pm$ 3.77 \\
            & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 10848.94} $\pm$ 2.52 \\
            & ER (m=5) & 5.53 $\pm$ 0.19 & 7098.58 $\pm$ 25.73 & 0.34 $\pm$ 0.14 & 10418.30 $\pm$ 6.35 \\
            & AGEM (m=5) & 4.94 $\pm$ 0.29 & 7025.89 $\pm$ 14.88 & 0.04 $\pm$ 0.11 & 10422.29 $\pm$ 3.88 \\
            & MT & 8.65 $\pm$ 0.78 & 7219.90 $\pm$ 94.54 & {\bf 1.56} $\pm$ 0.12 & 10406.50 $\pm$ 5.87 \\
            & FOMAML & {\bf 9.21} $\pm$ 0.10 & {\bf 7321.89} $\pm$ 24.02 & 1.55 $\pm$ 0.13 & 10365.44 $\pm$ 3.27 \\ \hline
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v2-results}
\end{table*}


\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
        & FT & -28.18 $\pm$ 2.39 & -12877.41 $\pm$ 809.17 & -29.01 $\pm$ 6.42 & -18087.20 $\pm$ 9708.56 \\
        & LP-FT & -29.50 $\pm$ 4.67 & -16359.04 $\pm$ 3416.32 & -3.39 $\pm$ 0.85 & -5459.86 $\pm$ 222.87 \\
        & ER (m=50) & -9.18 $\pm$ 1.20 & -11624.40 $\pm$ 178.76 & -7.15 $\pm$ 1.59 & -14715.09 $\pm$ 3321.96 \\
        & AGEM (m=50) & -13.77 $\pm$ 1.92 & -12160.87 $\pm$ 871.78 & -19.26 $\pm$ 4.04 & -18942.16 $\pm$ 10341.85 \\
        & MT & -3.88 $\pm$ 4.72 & -12087.56 $\pm$ 839.17 & -4.83 $\pm$ 4.48 & -12166.95 $\pm$ 1702.43 \\
        & FOMAML & -0.75 $\pm$ 1.12 & -11119.80 $\pm$ 435.87 & -1.40 $\pm$ 0.49 & -14680.75 $\pm$ 2735.12 \\ \hline
			 % \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 %& FT & -14.45 $\pm$ 0.82 & -7204.69 $\pm$ 62.66 & -13.51 $\pm$ 0.45 & -6123.39 $\pm$ 83.62 \\
    %         & LP-FT & -8.50 $\pm$ 0.76 & -7299.36 $\pm$ 26.00 & -2.66 $\pm$ 0.43 & -4717.24 $\pm$ 99.81 \\
    %         & ER (m=5) & -11.33 $\pm$ 1.44 & -7212.91 $\pm$ 41.46 & -11.36 $\pm$ 1.16 & -6043.47 $\pm$ 147.64 \\
    %         & AGEM (m=5) & -12.28 $\pm$ 0.67 & -7224.99 $\pm$ 51.53 & -12.11 $\pm$ 0.61 & -6133.68 $\pm$ 73.33 \\
    %         & MT & -1.30 $\pm$ 3.24 & -7160.07 $\pm$ 51.09 & -5.50 $\pm$ 2.94 & -6051.64 $\pm$ 88.90 \\
    %         & FOMAML & 1.99 $\pm$ 0.61 & -7137.91 $\pm$ 28.31 & -1.24 $\pm$ 0.35 & -5650.10 $\pm$ 90.00 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
		    & FT & -14.45 $\pm$ 0.82 & -7204.69 $\pm$ 62.66 & -13.51 $\pm$ 0.45 & -6123.39 $\pm$ 83.62 \\
            & LP-FT & -8.50 $\pm$ 0.76 & -7299.36 $\pm$ 26.00 & -2.66 $\pm$ 0.43 & -4717.24 $\pm$ 99.81 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & -7212.91 $\pm$ 41.46 & -11.36 $\pm$ 1.16 & -6043.47 $\pm$ 147.64 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & -7224.99 $\pm$ 51.53 & -12.11 $\pm$ 0.61 & -6133.68 $\pm$ 73.33 \\
            & MT & -1.30 $\pm$ 3.24 & -7160.07 $\pm$ 51.09 & -5.50 $\pm$ 2.94 & -6051.64 $\pm$ 88.90 \\
            & FOMAML & 1.99 $\pm$ 0.61 & -7137.91 $\pm$ 28.31 & -1.24 $\pm$ 0.35 & -5650.10 $\pm$ 90.00 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & -24279.86 $\pm$ 24.02 & 0.14 $\pm$ 0.34 & -23539.79 $\pm$ 28.40 \\
            & LP-FT & 1.18 $\pm$ 0.52 & -24304.66 $\pm$ 19.43 & 0.87 $\pm$ 0.09 & -23415.38 $\pm$ 15.09 \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & -24274.96 $\pm$ 10.16 & -0.05 $\pm$ 0.18 & -23524.10 $\pm$ 21.22 \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & -24291.05 $\pm$ 24.12 & -0.01 $\pm$ 0.15 & -23541.77 $\pm$ 11.61 \\
            & MT & 4.49 $\pm$ 0.80 & -24235.52 $\pm$ 18.47 & 0.77 $\pm$ 0.41 & -23493.29 $\pm$ 33.02 \\
            & FOMAML & 4.49 $\pm$ 0.45 & -24194.12 $\pm$ 11.36 & 0.84 $\pm$ 0.27 & -23497.38 $\pm$ 22.93 \\ \hline
% 			  \multirow{6}{0.12\linewidth}{CLEAR100} 
% 		    & FT & 5.06 $\pm$ 0.23 & 7030.61 $\pm$ 22.34 & -0.03 $\pm$ 0.11 & 10423.92 $\pm$ 3.77 \\
%             & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 10848.94} $\pm$ 2.52 \\
%             & ER (m=5) & 5.53 $\pm$ 0.19 & 7098.58 $\pm$ 25.73 & 0.34 $\pm$ 0.14 & 10418.30 $\pm$ 6.35 \\
%             & AGEM (m=5) & 4.94 $\pm$ 0.29 & 7025.89 $\pm$ 14.88 & 0.04 $\pm$ 0.11 & 10422.29 $\pm$ 3.88 \\
%             & MT & 8.65 $\pm$ 0.78 & 7219.90 $\pm$ 94.54 & {\bf 1.56} $\pm$ 0.12 & 10406.50 $\pm$ 5.87 \\
%             & FOMAML & {\bf 9.21} $\pm$ 0.10 & {\bf 7321.89} $\pm$ 24.02 & 1.55 $\pm$ 0.13 & 10365.44 $\pm$ 3.27 \\ \hline
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set with scaling of gram matrix. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v3-results}
\end{table*}



\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
            & FT & -28.18 $\pm$ 2.39 & 960.20 $\pm$ 156.14 & -29.01 $\pm$ 6.42 & 864.72 $\pm$ 475.06 \\
            & LP-FT & - & - & -3.39 $\pm$ 0.85 & {\bf 2666.60} $\pm$ 76.07 \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & 1182.18 $\pm$ 43.65 & -7.15 $\pm$ 1.59 & 1002.17 $\pm$ 449.25 \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & 1086.12 $\pm$ 152.66 & -19.26 $\pm$ 4.04 & 819.24 $\pm$ 583.73 \\
            & MT & -3.88 $\pm$ 4.72 & 1109.99 $\pm$ 138.92 & -4.83 $\pm$ 4.48 & 1296.58 $\pm$ 310.44 \\
            & FOMAML & {\bf -0.75} $\pm$ 1.12 & {\bf 1308.39} $\pm$ 91.54 & {\bf -1.40} $\pm$ 0.49 & 1023.42 $\pm$ 163.97 \\ \hline
			  \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 & FT & -25.83 $\pm$ 1.96 & 1470.31 $\pm$ 9.41 & -24.33 $\pm$ 3.38 & 1503.80 $\pm$ 89.12 \\
            & LP-FT & -23.93 $\pm$ 7.09 & 1408.53 $\pm$ 105.27 & -4.46 $\pm$ 0.37 & {\bf 1806.72} $\pm$ 3.14 \\
            & ER (m=20) & -9.44 $\pm$ 0.89 & 1511.31 $\pm$ 4.63 & -9.19 $\pm$ 0.23 & 1633.34 $\pm$ 11.29 \\
            & AGEM (m=20) & -18.70 $\pm$ 0.80 & 1474.74 $\pm$ 14.05 & -20.05 $\pm$ 2.52 & 1495.92 $\pm$ 53.66 \\
            & MT & -9.35 $\pm$ 3.99 & 1484.00 $\pm$ 18.67 & -7.93 $\pm$ 3.26 & 1598.35 $\pm$ 48.89 \\
            & FOMAML & {\bf -3.05} $\pm$ 0.79 & {\bf 1533.40} $\pm$ 8.16 & {\bf -4.40} $\pm$ 0.16 & 1659.53 $\pm$ 25.68 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
		    & FT & -14.45 $\pm$ 0.82 & 5327.33 $\pm$ 22.78 & -13.51 $\pm$ 0.45 & 5870.03 $\pm$ 36.55 \\
            & LP-FT & - & - & -2.66 $\pm$ 0.43 & {\bf 6523.80} $\pm$ 43.36 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & 5329.62 $\pm$ 15.70 & -11.36 $\pm$ 1.16 & 5906.27 $\pm$ 68.00 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & 5323.92 $\pm$ 20.54 & -12.11 $\pm$ 0.61 & 5861.62 $\pm$ 33.27 \\
            & MT & -1.30 $\pm$ 3.24 & 5352.62 $\pm$ 25.58 & -5.50 $\pm$ 2.94 & 5901.38 $\pm$ 41.72 \\
            & FOMAML & {\bf 1.99} $\pm$ 0.61 & {\bf 5366.34} $\pm$ 12.90 & {\bf -1.24} $\pm$ 0.35 & 6084.16 $\pm$ 39.42 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & 1063.00 $\pm$ 5.43 & 0.14 $\pm$ 0.34 & 1592.50 $\pm$ 2.76 \\
            & LP-FT & - & - & {\bf 0.87} $\pm$ 0.09 & {\bf 1625.92} $\pm$ 1.35 \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & 1063.93 $\pm$ 5.02 & -0.05 $\pm$ 0.18 & 1592.32 $\pm$ 1.62 \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & 1059.50 $\pm$ 6.15 & -0.01 $\pm$ 0.15 & 1594.12 $\pm$ 2.64 \\
            & MT & {\bf 4.49} $\pm$ 0.80 & {\bf 1074.85} $\pm$ 5.88 & 0.77 $\pm$ 0.41 & 1595.30 $\pm$ 2.66 \\
            & FOMAML & {\bf 4.49} $\pm$ 0.45 & 1072.77 $\pm$ 3.69 & 0.84 $\pm$ 0.27 & 1589.23 $\pm$ 1.67 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
            & FT & 5.06 $\pm$ 0.23 & 3830.14 $\pm$ 10.53 & -0.03 $\pm$ 0.11 & 5473.24 $\pm$ 1.81 \\
            & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 5683.37} $\pm$ 1.22 \\
            & ER (m=5) & 5.53 $\pm$ 0.19 & 3862.06 $\pm$ 12.11 & 0.34 $\pm$ 0.14 & 5470.71 $\pm$ 3.07 \\
            & AGEM (m=5) & 4.94 $\pm$ 0.29 & 3827.89 $\pm$ 6.97 & 0.04 $\pm$ 0.11 & 5472.47 $\pm$ 1.86 \\
            & MT & 8.65 $\pm$ 0.78 & 3919.56 $\pm$ 44.16 & {\bf 1.56} $\pm$ 0.12 & 5465.24 $\pm$ 2.80 \\
            & FOMAML & {\bf 9.21} $\pm$ 0.10 & {\bf 3967.18} $\pm$ 11.35 & 1.55 $\pm$ 0.13 & 5445.18 $\pm$ 1.61 \\ \hline
            \multirow{4}{0.12\linewidth}{Split ImageNet} 
    		& FT & -54.62 $\pm$ 1.82 & 1630.27 $\pm$ 2.12 & - & -\\
            & ER (m=10) & -27.56 $\pm$ 0.50 & 1764.60 $\pm$ 4.55 & - & - \\
            & AGEM (m=10) & -50.53 $\pm$ 1.27 & 1634.50 $\pm$ 3.47 & - & - \\
            & MT & -16.79 $\pm$ 0.56 & 1662.26 $\pm$ 2.65 & - & - \\ 
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set with scaling of gram matrix. We use diversity score from a paper. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v3-results}
\end{table*}


\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
            & FT & -28.18 $\pm$ 2.39 & 53.87 $\pm$ 10.26 & -29.01 $\pm$ 6.42 & 67.28 $\pm$ 35.72 \\
            & LP-FT & -29.50 $\pm$ 4.67 & 37.74 $\pm$ 18.06 & -3.39 $\pm$ 0.85 & {\bf 181.74} $\pm$ 13.96 \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & 58.60 $\pm$ 2.98 & -7.15 $\pm$ 1.59 & 73.61 $\pm$ 35.45 \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & 58.77 $\pm$ 10.22 & -19.26 $\pm$ 4.04 & 65.51 $\pm$ 43.39 \\
            & MT & -3.88 $\pm$ 4.72 & 60.38 $\pm$ 9.83 & -4.83 $\pm$ 4.48 & 96.03 $\pm$ 26.13 \\
            & FOMAML & {\bf -0.75} $\pm$ 1.12 & {\bf 63.10} $\pm$ 8.30 & {\bf -1.40} $\pm$ 0.49 & 71.18 $\pm$ 9.99 \\ \hline
			  \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 & FT & -25.83 $\pm$ 1.96 & 238.90 $\pm$ 1.48 & -24.33 $\pm$ 3.38 & 274.93 $\pm$ 22.34 \\
            & LP-FT & -23.93 $\pm$ 7.09 & 218.58 $\pm$ 18.36 & -4.46 $\pm$ 0.37 & 340.50 $\pm$ 2.34 \\
            & ER (m=20) & -9.44 $\pm$ 0.89 & 235.94 $\pm$ 0.71 & -9.19 $\pm$ 0.23 & 292.23 $\pm$ 3.22 \\
            & AGEM (m=20) & -18.70 $\pm$ 0.80 & 238.56 $\pm$ 1.62 & -20.05 $\pm$ 2.52 & 272.88 $\pm$ 15.31 \\
            & MT & -9.35 $\pm$ 3.99 & 238.06 $\pm$ 3.06 & -7.93 $\pm$ 3.26 & 289.25 $\pm$ 6.51 \\
            & FOMAML & {\bf -3.05} $\pm$ 0.79 & 234.99 $\pm$ 2.93 & -4.40 $\pm$ 0.16 & 286.07 $\pm$ 7.55 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
		    & FT & -14.45 $\pm$ 0.82 & 473.70 $\pm$ 2.54 & -13.51 $\pm$ 0.45 & 613.87 $\pm$ 9.63 \\
            & LP-FT & -8.50 $\pm$ 0.76 & 462.91 $\pm$ 3.54 & -2.66 $\pm$ 0.43 & 712.37 $\pm$ 2.30 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & 473.71 $\pm$ 3.58 & -11.36 $\pm$ 1.16 & 612.42 $\pm$ 16.54 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & 472.40 $\pm$ 3.79 & -12.11 $\pm$ 0.61 & 610.64 $\pm$ 13.80 \\
            & MT & -1.30 $\pm$ 3.24 & 476.25 $\pm$ 3.27 & -5.50 $\pm$ 2.94 & 615.19 $\pm$ 9.52 \\
            & FOMAML & 1.99 $\pm$ 0.61 & 474.47 $\pm$ 3.69 & -1.24 $\pm$ 0.35 & 632.77 $\pm$ 5.03 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & 77.86 $\pm$ 1.28 & 0.14 $\pm$ 0.34 & 267.91 $\pm$ 0.98 \\
            & LP-FT & 1.18 $\pm$ 0.52 & 78.87 $\pm$ 1.12 & 0.87 $\pm$ 0.09 & 287.85 $\pm$ 0.26 \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & 78.07 $\pm$ 1.28 & -0.05 $\pm$ 0.18 & 266.08 $\pm$ 0.54 \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & 77.19 $\pm$ 1.39 & -0.01 $\pm$ 0.15 & 268.48 $\pm$ 0.93 \\
            & MT & 4.49 $\pm$ 0.80 & 80.27 $\pm$ 1.01 & 0.77 $\pm$ 0.41 & 267.44 $\pm$ 1.18 \\
            & FOMAML & 4.49 $\pm$ 0.45 & 79.29 $\pm$ 0.94 & 0.84 $\pm$ 0.27 & 265.14 $\pm$ 0.96 \\ \hline
			 % \multirow{6}{0.12\linewidth}{CLEAR100} 
    %         & FT & 5.06 $\pm$ 0.23 & 3830.14 $\pm$ 10.53 & -0.03 $\pm$ 0.11 & 5473.24 $\pm$ 1.81 \\
    %         & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 5683.37} $\pm$ 1.22 \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 3862.06 $\pm$ 12.11 & 0.34 $\pm$ 0.14 & 5470.71 $\pm$ 3.07 \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 3827.89 $\pm$ 6.97 & 0.04 $\pm$ 0.11 & 5472.47 $\pm$ 1.86 \\
    %         & MT & 8.65 $\pm$ 0.78 & 3919.56 $\pm$ 44.16 & {\bf 1.56} $\pm$ 0.12 & 5465.24 $\pm$ 2.80 \\
    %         & FOMAML & {\bf 9.21} $\pm$ 0.10 & {\bf 3967.18} $\pm$ 11.35 & 1.55 $\pm$ 0.13 & 5445.18 $\pm$ 1.61 \\ \hline
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set with scaling of gram matrix. Use l2 normalization. We use diversity score from a paper. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v4-results}
\end{table*}


\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
            & FT & -28.18 $\pm$ 2.39 & 0.15 $\pm$ 0.01 & -29.01 $\pm$ 6.42 & 0.17 $\pm$ 0.06 \\
            & LP-FT & -29.50 $\pm$ 4.67 & 0.17 $\pm$ 0.06 & -3.39 $\pm$ 0.85 & 0.11 $\pm$ 0.01 \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & 0.16 $\pm$ 0.02 & -7.15 $\pm$ 1.59 & 0.17 $\pm$ 0.06 \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & 0.16 $\pm$ 0.04 & -19.26 $\pm$ 4.04 & 0.18 $\pm$ 0.08 \\
            & MT & -3.88 $\pm$ 4.72 & 0.16 $\pm$ 0.04 & -4.83 $\pm$ 4.48 & 0.14 $\pm$ 0.04 \\
            & FOMAML & -0.75 $\pm$ 1.12 & 0.14 $\pm$ 0.03 & -1.40 $\pm$ 0.49 & 0.15 $\pm$ 0.04 \\ \hline
			 % \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 %& FT & -25.83 $\pm$ 1.96 & 238.90 $\pm$ 1.48 & -24.33 $\pm$ 3.38 & 274.93 $\pm$ 22.34 \\
    %         & LP-FT & -23.93 $\pm$ 7.09 & 218.58 $\pm$ 18.36 & -4.46 $\pm$ 0.37 & 340.50 $\pm$ 2.34 \\
    %         & ER (m=20) & -9.44 $\pm$ 0.89 & 235.94 $\pm$ 0.71 & -9.19 $\pm$ 0.23 & 292.23 $\pm$ 3.22 \\
    %         & AGEM (m=20) & -18.70 $\pm$ 0.80 & 238.56 $\pm$ 1.62 & -20.05 $\pm$ 2.52 & 272.88 $\pm$ 15.31 \\
    %         & MT & -9.35 $\pm$ 3.99 & 238.06 $\pm$ 3.06 & -7.93 $\pm$ 3.26 & 289.25 $\pm$ 6.51 \\
    %         & FOMAML & {\bf -3.05} $\pm$ 0.79 & 234.99 $\pm$ 2.93 & -4.40 $\pm$ 0.16 & 286.07 $\pm$ 7.55 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
    		 & FT & -14.45 $\pm$ 0.82 & 0.42 $\pm$ 0.03 & -13.51 $\pm$ 0.45 & 0.32 $\pm$ 0.02 \\
            & LP-FT & -8.50 $\pm$ 0.76 & 0.43 $\pm$ 0.01 & -2.66 $\pm$ 0.43 & 0.27 $\pm$ 0.01 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & 0.41 $\pm$ 0.01 & -11.36 $\pm$ 1.16 & 0.32 $\pm$ 0.02 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & 0.42 $\pm$ 0.01 & -12.11 $\pm$ 0.61 & 0.32 $\pm$ 0.02 \\
            & MT & -1.30 $\pm$ 3.24 & 0.41 $\pm$ 0.01 & -5.50 $\pm$ 2.94 & 0.32 $\pm$ 0.02 \\
            & FOMAML & 1.99 $\pm$ 0.61 & 0.42 $\pm$ 0.01 & -1.24 $\pm$ 0.35 & 0.32 $\pm$ 0.02 \\ \hline
			 % \multirow{6}{0.12\linewidth}{CLEAR10} 
			 %& FT & 0.93 $\pm$ 0.82 & 77.86 $\pm$ 1.28 & 0.14 $\pm$ 0.34 & 267.91 $\pm$ 0.98 \\
    %         & LP-FT & 1.18 $\pm$ 0.52 & 78.87 $\pm$ 1.12 & 0.87 $\pm$ 0.09 & 287.85 $\pm$ 0.26 \\
    %         & ER (m=10) & 1.79 $\pm$ 0.19 & 78.07 $\pm$ 1.28 & -0.05 $\pm$ 0.18 & 266.08 $\pm$ 0.54 \\
    %         & AGEM (m=10) & 2.03 $\pm$ 0.69 & 77.19 $\pm$ 1.39 & -0.01 $\pm$ 0.15 & 268.48 $\pm$ 0.93 \\
    %         & MT & 4.49 $\pm$ 0.80 & 80.27 $\pm$ 1.01 & 0.77 $\pm$ 0.41 & 267.44 $\pm$ 1.18 \\
    %         & FOMAML & 4.49 $\pm$ 0.45 & 79.29 $\pm$ 0.94 & 0.84 $\pm$ 0.27 & 265.14 $\pm$ 0.96 \\ \hline
			 % \multirow{6}{0.12\linewidth}{CLEAR100} 
    %         & FT & 5.06 $\pm$ 0.23 & 3830.14 $\pm$ 10.53 & -0.03 $\pm$ 0.11 & 5473.24 $\pm$ 1.81 \\
    %         & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 5683.37} $\pm$ 1.22 \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 3862.06 $\pm$ 12.11 & 0.34 $\pm$ 0.14 & 5470.71 $\pm$ 3.07 \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 3827.89 $\pm$ 6.97 & 0.04 $\pm$ 0.11 & 5472.47 $\pm$ 1.86 \\
    %         & MT & 8.65 $\pm$ 0.78 & 3919.56 $\pm$ 44.16 & {\bf 1.56} $\pm$ 0.12 & 5465.24 $\pm$ 2.80 \\
    %         & FOMAML & {\bf 9.21} $\pm$ 0.10 & {\bf 3967.18} $\pm$ 11.35 & 1.55 $\pm$ 0.13 & 5445.18 $\pm$ 1.61 \\ \hline
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set with scaling of gram matrix. Use normalization. We use diversity score from a paper. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-nuclear-results}
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			\multirow{6}{0.12\linewidth}{Split CIFAR-10}
            & FT & -28.18 $\pm$ 2.39 & 35.59 $\pm$ 8.47 & -29.01 $\pm$ 6.42 & 60.18 $\pm$ 29.28 \\
            & LP-FT & - & - & -3.39 $\pm$ 0.85 & {\bf 171.41} $\pm$ 10.80 \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & 37.33 $\pm$ 11.81 & -7.15 $\pm$ 1.59 & 66.18 $\pm$ 28.79 \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & 35.79 $\pm$ 13.16 & -19.26 $\pm$ 4.04 & 60.77 $\pm$ 33.67 \\
            & MT & -3.88 $\pm$ 4.72 & 36.88 $\pm$ 10.64 & -4.83 $\pm$ 4.48 & 86.88 $\pm$ 17.57 \\
            & FOMAML & {\bf -0.75} $\pm$ 1.12 & {\bf 45.52} $\pm$ 6.30 & -1.40 $\pm$ 0.49 & 65.26 $\pm$ 8.35 \\ \hline
			  \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			& FT & -25.83 $\pm$ 1.96 & 224.27 $\pm$ 2.92 & -24.33 $\pm$ 3.38 & 263.31 $\pm$ 22.12 \\
            & LP-FT & - & - & -4.46 $\pm$ 0.37 & {\bf 332.10} $\pm$ 2.39 \\
            & ER (m=20) & -9.44 $\pm$ 0.89 & 225.95 $\pm$ 1.92 & -9.19 $\pm$ 0.23 & 281.31 $\pm$ 2.89 \\
            & AGEM (m=20) & -18.70 $\pm$ 0.80 & 224.46 $\pm$ 2.36 & -20.05 $\pm$ 2.52 & 260.01 $\pm$ 16.37 \\
            & MT & -9.35 $\pm$ 3.99 & 225.33 $\pm$ 3.72 & -7.93 $\pm$ 3.26 & 277.14 $\pm$ 6.69 \\
            & FOMAML & {\bf -3.05} $\pm$ 0.79 & 225.87 $\pm$ 4.28 & -4.40 $\pm$ 0.16 & 271.56 $\pm$ 6.00 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR-100 Superclasses} 
    		 & FT & -14.45 $\pm$ 0.82 & 458.73 $\pm$ 10.46 & -13.51 $\pm$ 0.45 & 599.29 $\pm$ 10.99 \\
            & LP-FT & - & - & -2.66 $\pm$ 0.43 & {\bf 702.43} $\pm$ 3.30 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & 463.78 $\pm$ 6.33 & -11.36 $\pm$ 1.16 & 600.23 $\pm$ 19.21 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & 459.65 $\pm$ 11.69 & -12.11 $\pm$ 0.61 & 594.70 $\pm$ 22.15 \\
            & MT & -1.30 $\pm$ 3.24 & 465.47 $\pm$ 6.31 & -5.50 $\pm$ 2.94 & 601.38 $\pm$ 13.63 \\
            & FOMAML & {\bf 1.99} $\pm$ 0.61 & {\bf 470.27} $\pm$ 4.17 & -1.24 $\pm$ 0.35 & 620.66 $\pm$ 8.33 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & 76.72 $\pm$ 1.37 & 0.14 $\pm$ 0.34 & 265.72 $\pm$ 0.87 \\
            & LP-FT & - & - & 0.87 $\pm$ 0.09 & {\bf 281.78} $\pm$ 0.27 \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & 76.76 $\pm$ 1.31 & -0.05 $\pm$ 0.18 & 263.89 $\pm$ 0.66 \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & 76.00 $\pm$ 1.44 & -0.01 $\pm$ 0.15 & 266.36 $\pm$ 0.82 \\
            & MT & {\bf 4.49} $\pm$ 0.80 & {\bf 79.01} $\pm$ 1.14 & 0.77 $\pm$ 0.41 & 265.25 $\pm$ 1.20 \\
            & FOMAML & {\bf 4.49} $\pm$ 0.45 & 77.98 $\pm$ 1.02 & 0.84 $\pm$ 0.27 & 262.88 $\pm$ 1.03 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
            & FT & 5.06 $\pm$ 0.23 & 179.47 $\pm$ 0.82 & -0.03 $\pm$ 0.11 & 441.22 $\pm$ 0.40 \\
            & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 488.94} $\pm$ 0.58 \\
            & ER (m=5) & 5.53 $\pm$ 0.19 & 181.39 $\pm$ 1.26 & 0.34 $\pm$ 0.14 & 440.48 $\pm$ 0.64 \\
            & AGEM (m=5) & 4.94 $\pm$ 0.29 & 179.12 $\pm$ 0.83 & 0.04 $\pm$ 0.11 & 441.26 $\pm$ 0.22 \\
            & MT & 8.65 $\pm$ 0.78 & {\bf 186.16} $\pm$ 2.67 & 1.56 $\pm$ 0.12 & 444.38 $\pm$ 0.33 \\
            & FOMAML & {\bf 9.21} $\pm$ 0.10 & 184.38 $\pm$ 1.27 & 1.55 $\pm$ 0.13 & 440.30 $\pm$ 0.57 \\ 
    %         \multirow{4}{0.12\linewidth}{Split ImageNet} 
			 %& FT & -54.62 $\pm$ 1.82 & 271.98 $\pm$ 0.78 & - &  - \\
    %         & ER (m=10) & -27.56 $\pm$ 0.50 & 289.18 $\pm$ 3.21 & - & - \\
    %         & AGEM (m=10) & -50.53 $\pm$ 1.27 & 274.07 $\pm$ 0.97 & - & - \\
    %         & MT & -16.79 $\pm$ 0.56 & 274.88 $\pm$ 1.72 & - & - \\ 
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set with scaling of gram matrix. Use frobenius normalization. We use diversity score from a paper. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v5-results}
\end{table*}



\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
& FT & -28.18 $\pm$ 2.39 & 436.52 $\pm$ 53.18 & -29.01 $\pm$ 6.42 & 440.99 $\pm$ 179.81 \\
& LP-FT & -29.50 $\pm$ 4.67 & 332.37 $\pm$ 114.08 & -3.39 $\pm$ 0.85 & 937.49 $\pm$ 19.28 \\
& ER (m=50) & -9.18 $\pm$ 1.20 & 457.78 $\pm$ 25.99 & -7.15 $\pm$ 1.59 & 491.85 $\pm$ 85.68 \\
& AGEM (m=50) & -13.77 $\pm$ 1.92 & 458.26 $\pm$ 43.57 & -19.26 $\pm$ 4.04 & 439.72 $\pm$ 178.48 \\
& MT & -3.88 $\pm$ 4.72 & 465.63 $\pm$ 27.17 & -4.83 $\pm$ 4.48 & 582.46 $\pm$ 57.31 \\
& FOMAML & -0.75 $\pm$ 1.12 & 479.56 $\pm$ 7.77 & -1.40 $\pm$ 0.49 & 481.29 $\pm$ 101.63 \\ \hline
			  \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 & FT & -25.83 $\pm$ 1.96 & 407.54 $\pm$ 1.93 & -24.33 $\pm$ 3.38 & 453.27 $\pm$ 27.51 \\
& LP-FT & -23.93 $\pm$ 7.09 & 382.43 $\pm$ 23.39 & -4.46 $\pm$ 0.37 & 532.70 $\pm$ 3.27 \\
& ER (m=20) & -9.44 $\pm$ 0.89 & 403.69 $\pm$ 0.93 & -9.19 $\pm$ 0.23 & 473.38 $\pm$ 4.27 \\
& AGEM (m=20) & -18.70 $\pm$ 0.80 & 407.02 $\pm$ 2.15 & -20.05 $\pm$ 2.52 & 450.71 $\pm$ 18.87 \\
& MT & -9.35 $\pm$ 3.99 & 406.21 $\pm$ 3.99 & -7.93 $\pm$ 3.26 & 469.58 $\pm$ 8.35 \\
& FOMAML & -3.05 $\pm$ 0.79 & 402.78 $\pm$ 3.90 & -4.40 $\pm$ 0.16 & 465.63 $\pm$ 9.56 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
		& FT & -14.45 $\pm$ 0.82 & 648.06 $\pm$ 4.16 & -13.51 $\pm$ 0.45 & 797.52 $\pm$ 14.40 \\
& LP-FT & -8.50 $\pm$ 0.76 & 637.09 $\pm$ 4.43 & -2.66 $\pm$ 0.43 & 905.41 $\pm$ 3.16 \\
& ER (m=5) & -11.33 $\pm$ 1.44 & 648.35 $\pm$ 4.28 & -11.36 $\pm$ 1.16 & 796.09 $\pm$ 21.80 \\
& AGEM (m=5) & -12.28 $\pm$ 0.67 & 646.68 $\pm$ 5.79 & -12.11 $\pm$ 0.61 & 793.86 $\pm$ 19.47 \\
& MT & -1.30 $\pm$ 3.24 & 650.99 $\pm$ 3.79 & -5.50 $\pm$ 2.94 & 798.74 $\pm$ 13.99 \\
& FOMAML & 1.99 $\pm$ 0.61 & 650.19 $\pm$ 4.63 & -1.24 $\pm$ 0.35 & 819.00 $\pm$ 7.40 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			& FT & 0.93 $\pm$ 0.82 & 141.55 $\pm$ 1.74 & 0.14 $\pm$ 0.34 & 361.77 $\pm$ 1.16 \\
& LP-FT & 1.18 $\pm$ 0.52 & 142.74 $\pm$ 1.61 & 0.87 $\pm$ 0.09 & 384.65 $\pm$ 0.31 \\
& ER (m=10) & 1.79 $\pm$ 0.19 & 141.59 $\pm$ 1.78 & -0.05 $\pm$ 0.18 & 359.63 $\pm$ 0.67 \\
& AGEM (m=10) & 2.03 $\pm$ 0.69 & 140.66 $\pm$ 1.80 & -0.01 $\pm$ 0.15 & 362.44 $\pm$ 1.10 \\
& MT & 4.49 $\pm$ 0.80 & 144.17 $\pm$ 1.28 & 0.77 $\pm$ 0.41 & 361.23 $\pm$ 1.40 \\
& FOMAML & 4.49 $\pm$ 0.45 & 142.99 $\pm$ 1.25 & 0.84 $\pm$ 0.27 & 358.75 $\pm$ 1.07 \\ \hline
			 % \multirow{6}{0.12\linewidth}{CLEAR100} 
    %         & FT & 5.06 $\pm$ 0.23 & 3830.14 $\pm$ 10.53 & -0.03 $\pm$ 0.11 & 5473.24 $\pm$ 1.81 \\
    %         & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 5683.37} $\pm$ 1.22 \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 3862.06 $\pm$ 12.11 & 0.34 $\pm$ 0.14 & 5470.71 $\pm$ 3.07 \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 3827.89 $\pm$ 6.97 & 0.04 $\pm$ 0.11 & 5472.47 $\pm$ 1.86 \\
    %         & MT & 8.65 $\pm$ 0.78 & 3919.56 $\pm$ 44.16 & {\bf 1.56} $\pm$ 0.12 & 5465.24 $\pm$ 2.80 \\
    %         & FOMAML & {\bf 9.21} $\pm$ 0.10 & {\bf 3967.18} $\pm$ 11.35 & 1.55 $\pm$ 0.13 & 5445.18 $\pm$ 1.61 \\ \hline
    %         \multirow{6}{0.12\linewidth}{Split ImageNet} 
			 %& FT & 5.06 $\pm$ 0.23 & 27.81 $\pm$ 0.28 & -0.03 $\pm$ 0.11 & 79.99 $\pm$ 0.11  \\
    %         & LP-FT & 5.13 $\pm$ 0.47 & 29.08 $\pm$ 0.27 & 1.52 $\pm$ 0.06 & 82.20 $\pm$ 0.04  \\
    %         & MT & 8.65 $\pm$ 0.78 & 31.03 $\pm$ 0.54 & 1.56 $\pm$ 0.12 & 82.13 $\pm$ 0.10  \\
    %         & ER (m=5) & 5.53 $\pm$ 0.19 & 27.70 $\pm$ 0.27 & 0.34 $\pm$ 0.14 & 80.41 $\pm$ 0.09  \\
    %         & AGEM (m=5) & 4.94 $\pm$ 0.29 & 27.64 $\pm$ 0.27 & 0.04 $\pm$ 0.11 & 79.96 $\pm$ 0.04  \\
    %         & FOMAML & 9.21 $\pm$ 0.10 & 32.07 $\pm$ 0.37 & 1.55 $\pm$ 0.13 & 81.99 $\pm$ 0.14  \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set with scaling of gram matrix. Use l2 normalization. score 1. We use diversity score from a paper. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v4-results}
\end{table*}


\begin{table*}[htb]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt$ & $\avgfdiv$ &   $\avgfgt$ & $\avgfdiv$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
            & FT & -28.18 $\pm$ 2.39 & 559.31 $\pm$ 109.11 & -29.01 $\pm$ 6.42 & 667.05 $\pm$ 331.13 \\
            & LP-FT & - & - & -3.39 $\pm$ 0.85 & {\bf 1464.10} $\pm$ 35.85 \\
            & ER (m=50) & -9.18 $\pm$ 1.20 & 576.51 $\pm$ 169.18 & -7.15 $\pm$ 1.59 & 725.55 $\pm$ 220.18 \\
            & AGEM (m=50) & -13.77 $\pm$ 1.92 & 523.85 $\pm$ 128.53 & -19.26 $\pm$ 4.04 & 643.80 $\pm$ 367.81 \\
            & MT & -3.88 $\pm$ 4.72 & 557.19 $\pm$ 106.69 & -4.83 $\pm$ 4.48 & 945.24 $\pm$ 100.12 \\
            & FOMAML & {\bf -0.75} $\pm$ 1.12 & {\bf 691.39} $\pm$ 80.19 & -1.40 $\pm$ 0.49 & 755.20 $\pm$ 89.42 \\ \hline
			  \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
			 & FT & -25.83 $\pm$ 1.96 & 1046.07 $\pm$ 6.77 & -24.33 $\pm$ 3.38 & 1098.88 $\pm$ 42.55 \\
            & LP-FT & - & - & -4.46 $\pm$ 0.37 & {\bf 1203.71} $\pm$ 3.42 \\
            & ER (m=20) & -9.44 $\pm$ 0.89 & 1046.87 $\pm$ 7.91 & -9.19 $\pm$ 0.23 & 1129.53 $\pm$ 4.57 \\
            & AGEM (m=20) & -18.70 $\pm$ 0.80 & 1048.53 $\pm$ 6.25 & -20.05 $\pm$ 2.52 & 1090.22 $\pm$ 32.33 \\
            & MT & -9.35 $\pm$ 3.99 & 1049.78 $\pm$ 5.56 & -7.93 $\pm$ 3.26 & 1122.01 $\pm$ 10.67 \\
            & FOMAML & {\bf -3.05} $\pm$ 0.79 & 1049.69 $\pm$ 9.18 & -4.40 $\pm$ 0.16 & 1113.15 $\pm$ 10.10 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR100 Superclasses} 
    		& FT & -14.45 $\pm$ 0.82 & 3255.63 $\pm$ 60.07 & -13.51 $\pm$ 0.45 & 3588.18 $\pm$ 44.21 \\
            & LP-FT & - & - & -2.66 $\pm$ 0.43 & {\bf 3870.26} $\pm$ 8.98 \\
            & ER (m=5) & -11.33 $\pm$ 1.44 & 3280.94 $\pm$ 26.89 & -11.36 $\pm$ 1.16 & 3593.19 $\pm$ 64.70 \\
            & AGEM (m=5) & -12.28 $\pm$ 0.67 & 3264.90 $\pm$ 53.59 & -12.11 $\pm$ 0.61 & 3571.20 $\pm$ 78.76 \\
            & MT & -1.30 $\pm$ 3.24 & 3285.54 $\pm$ 25.19 & -5.50 $\pm$ 2.94 & 3589.98 $\pm$ 44.77 \\
            & FOMAML & {\bf 1.99} $\pm$ 0.61 & {\bf 3303.66} $\pm$ 14.02 & -1.24 $\pm$ 0.35 & 3646.64 $\pm$ 29.43 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & 770.55 $\pm$ 4.53 & 0.14 $\pm$ 0.34 & 1175.98 $\pm$ 1.72 \\
            & LP-FT & - & - & 0.87 $\pm$ 0.09 & {\bf 1197.19} $\pm$ 0.51 \\
            & ER (m=10) & 1.79 $\pm$ 0.19 & 770.67 $\pm$ 4.48 & -0.05 $\pm$ 0.18 & 1172.77 $\pm$ 1.17 \\
            & AGEM (m=10) & 2.03 $\pm$ 0.69 & 767.45 $\pm$ 4.90 & -0.01 $\pm$ 0.15 & 1177.08 $\pm$ 1.35 \\
            & MT & {\bf 4.49} $\pm$ 0.80 & {\bf 782.20} $\pm$ 5.50 & 0.77 $\pm$ 0.41 & 1174.83 $\pm$ 2.21 \\
            & FOMAML & {\bf 4.49} $\pm$ 0.45 & 774.18 $\pm$ 3.68 & 0.84 $\pm$ 0.27 & 1171.44 $\pm$ 1.48 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
            & FT & 5.06 $\pm$ 0.23 & 2344.81 $\pm$ 6.86 & -0.03 $\pm$ 0.11 & 3373.05 $\pm$ 2.11 \\
            & LP-FT & - & - & 1.52 $\pm$ 0.06 & {\bf 3532.43} $\pm$ 1.85 \\
            & ER (m=5) & 5.53 $\pm$ 0.19 & 2366.39 $\pm$ 10.53 & 0.34 $\pm$ 0.14 & 3370.42 $\pm$ 2.57 \\
            & AGEM (m=5) & 4.94 $\pm$ 0.29 & 2342.38 $\pm$ 5.59 & 0.04 $\pm$ 0.11 & 3373.00 $\pm$ 0.74 \\
            & MT & 8.65 $\pm$ 0.78 & {\bf 2402.52} $\pm$ 17.46 & 1.56 $\pm$ 0.12 & 3393.40 $\pm$ 1.44 \\
            & FOMAML & {\bf 9.21} $\pm$ 0.10 & 2384.39 $\pm$ 9.55 & 1.55 $\pm$ 0.13 & 3380.30 $\pm$ 2.32 \\ \hline
            \multirow{6}{0.12\linewidth}{Split ImageNet} 
			& FT & -54.62 $\pm$ 1.82 & 1208.06 $\pm$ 1.08 & - & - \\
            & ER (m=10) & -27.56 $\pm$ 0.50 & 1231.90 $\pm$ 4.88 & - & - \\
            & AGEM (m=10) & -50.53 $\pm$ 1.27 & 1211.28 $\pm$ 1.49 & - & - \\
            & MT & -16.79 $\pm$ 0.56 & 1211.95 $\pm$ 2.57 & - & - \\ 
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Calculate $\avgfdiv$ using the entire test set with scaling of gram matrix. Use frobenius normalization. $\epsilon=0.05$. We use diversity score from a paper. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v5-results}
\end{table*}


\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
		\begin{tabular}{l|l|cc|cc}
			\toprule
			  \multirow{2}{0.12\linewidth}{Dataset} &  \multirow{2}{0.08\linewidth}{Method} &   \multicolumn{2}{c}{Random Init} & \multicolumn{2}{c}{Pre-trained}   \\ \cline{3-6}
			  & & $\avgfgt \uparrow$ & $\avgfdiv \uparrow$ &   $\avgfgt \uparrow$ & $\avgfdiv \uparrow$ \\ \hline
			 \multirow{6}{0.12\linewidth}{Split CIFAR-10}
            & FT & -28.18 $\pm$ 2.39 & 1.18 $\pm$ 0.04 & -29.01 $\pm$ 6.42 & 1.19 $\pm$ 0.06 \\
& LP-FT & -29.50 $\pm$ 4.67 & 1.18 $\pm$ 0.07 & -3.39 $\pm$ 0.85 & 1.24 $\pm$ 0.02 \\
& ER (m=50) & -9.18 $\pm$ 1.20 & 1.17 $\pm$ 0.02 & -7.15 $\pm$ 1.59 & 1.17 $\pm$ 0.07 \\
& AGEM (m=50) & -13.77 $\pm$ 1.92 & 1.17 $\pm$ 0.08 & -19.26 $\pm$ 4.04 & 1.18 $\pm$ 0.06 \\
& MT & -3.88 $\pm$ 4.72 & 1.18 $\pm$ 0.07 & -4.83 $\pm$ 4.48 & 1.20 $\pm$ 0.06 \\
& FOMAML & -0.75 $\pm$ 1.12 & 1.19 $\pm$ 0.06 & -1.40 $\pm$ 0.49 & 1.19 $\pm$ 0.06 \\ \hline
			  \multirow{6}{0.12\linewidth}{Split CIFAR-100} 
		& FT & -25.83 $\pm$ 1.96 & 2.38 $\pm$ 0.01 & -24.33 $\pm$ 3.38 & 2.51 $\pm$ 0.09 \\
& LP-FT & -23.93 $\pm$ 7.09 & 2.30 $\pm$ 0.09 & -4.46 $\pm$ 0.37 & 2.75 $\pm$ 0.01 \\
& ER (m=20) & -9.44 $\pm$ 0.89 & 2.38 $\pm$ 0.01 & -9.19 $\pm$ 0.23 & 2.58 $\pm$ 0.01 \\
& AGEM (m=20) & -18.70 $\pm$ 0.80 & 2.38 $\pm$ 0.01 & -20.05 $\pm$ 2.52 & 2.50 $\pm$ 0.06 \\
& MT & -9.35 $\pm$ 3.99 & 2.38 $\pm$ 0.02 & -7.93 $\pm$ 3.26 & 2.57 $\pm$ 0.02 \\
& FOMAML & -3.05 $\pm$ 0.79 & 2.37 $\pm$ 0.01 & -4.40 $\pm$ 0.16 & 2.55 $\pm$ 0.02 \\ \hline
			  \multirow{6}{0.12\linewidth}{CIFAR-100 Superclasses} 
    		& FT & -14.45 $\pm$ 0.82 & 3.69 $\pm$ 0.02 & -13.51 $\pm$ 0.45 & 4.30 $\pm$ 0.04 \\
& LP-FT & -8.50 $\pm$ 0.76 & 3.64 $\pm$ 0.02 & -2.66 $\pm$ 0.43 & 4.68 $\pm$ 0.04 \\
& ER (m=5) & -11.33 $\pm$ 1.44 & 3.69 $\pm$ 0.03 & -11.36 $\pm$ 1.16 & 4.30 $\pm$ 0.04 \\
& AGEM (m=5) & -12.28 $\pm$ 0.67 & 3.68 $\pm$ 0.02 & -12.11 $\pm$ 0.61 & 4.29 $\pm$ 0.02 \\
& MT & -1.30 $\pm$ 3.24 & 3.70 $\pm$ 0.03 & -5.50 $\pm$ 2.94 & 4.31 $\pm$ 0.03 \\
& FOMAML & 1.99 $\pm$ 0.61 & 3.69 $\pm$ 0.02 & -1.24 $\pm$ 0.35 & 4.37 $\pm$ 0.04 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR10} 
			 & FT & 0.93 $\pm$ 0.82 & 2.22 $\pm$ 0.01 & 0.14 $\pm$ 0.34 & 3.85 $\pm$ 0.00 \\
& LP-FT & 1.18 $\pm$ 0.52 & 2.22 $\pm$ 0.01 & 0.87 $\pm$ 0.09 & 3.97 $\pm$ 0.00 \\
& ER (m=10) & 1.79 $\pm$ 0.19 & 2.22 $\pm$ 0.01 & -0.05 $\pm$ 0.18 & 3.84 $\pm$ 0.00 \\
& AGEM (m=10) & 2.03 $\pm$ 0.69 & 2.21 $\pm$ 0.02 & -0.01 $\pm$ 0.15 & 3.85 $\pm$ 0.00 \\
& MT & 4.49 $\pm$ 0.80 & 2.25 $\pm$ 0.01 & 0.77 $\pm$ 0.41 & 3.85 $\pm$ 0.01 \\
& FOMAML & 4.49 $\pm$ 0.45 & 2.24 $\pm$ 0.01 & 0.84 $\pm$ 0.27 & 3.83 $\pm$ 0.01 \\ \hline
			  \multirow{6}{0.12\linewidth}{CLEAR100} 
           & FT & 5.06 $\pm$ 0.23 & 3.23 $\pm$ 0.01 & -0.03 $\pm$ 0.11 & 6.04 $\pm$ 0.00 \\
& LP-FT & 5.13 $\pm$ 0.47 & 3.38 $\pm$ 0.01 & 1.52 $\pm$ 0.06 & 6.57 $\pm$ 0.01 \\
& ER (m=5) & 5.53 $\pm$ 0.19 & 3.25 $\pm$ 0.01 & 0.34 $\pm$ 0.14 & 6.04 $\pm$ 0.01 \\
& AGEM (m=5) & 4.94 $\pm$ 0.29 & 3.23 $\pm$ 0.01 & 0.04 $\pm$ 0.11 & 6.04 $\pm$ 0.01 \\
& MT & 8.65 $\pm$ 0.78 & 3.30 $\pm$ 0.02 & 1.56 $\pm$ 0.12 & 6.07 $\pm$ 0.00 \\
& FOMAML & 9.21 $\pm$ 0.10 & 3.28 $\pm$ 0.01 & 1.55 $\pm$ 0.13 & 6.03 $\pm$ 0.01 \\ \hline
             \multirow{5}{0.12\linewidth}{Split ImageNet} 
            & FT & -54.62 $\pm$ 1.82 & 3.63 $\pm$ 0.01 & - & - \\
& LP-FT & -49.08 $\pm$ 1.71 & 3.81 $\pm$ 0.02 & - & -  \\
& ER (m=10) & -27.56 $\pm$ 0.50 & 3.72 $\pm$ 0.02 & - & -  \\
& AGEM (m=10) & -50.53 $\pm$ 1.27 & 3.65 $\pm$ 0.01 & - & -  \\
& MT & -16.79 $\pm$ 0.56 & 3.67 $\pm$ 0.01 & - & -  \\
& FOMAML & -10.58 $\pm$ 0.55 & 3.88 $\pm$ 0.03 & - & -  \\ 
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small Comparing $\avgfgt$ with $\avgfdiv$. The numbers for $\avgfgt$ are percentages. {\bf Bold} numbers are superior results. }
	\label{tab:feature-score-v2-results}
	\negspace{-5mm}
\end{table*}
